Capturing Periodic I/O Using Frequency Techniques

Many HPC applications perform their I/O in bursts that follow a periodic pattern. This allows for making predictions as to when a burst occurs. System providers can take advantage of such knowledge to reduce file-system contention by actively scheduling I/O bandwidth. The effectiveness of this approach, however, depends on the ability to detect and quantify the periodicity of I/O patterns online. In this paper, we introduce FTIO, an online method to detect periodic I/O phases, which is based on discrete Fourier transform (DFT), combined with outlier detection. We provide metrics that gauge the confidence in the output and tell how far from being periodic the signal is. We validate our approach with large-scale experiments on a production system and examine its limitations extensively. Our experiments show that FTIO has a mean error below 11%. Finally, we demonstrate that FTIO allowed the I/O scheduler Set- 10 to boost system utilization by 26% and reduce I/O slowdown by 56%.

==> Makefile <==
BASENAME = main

all: pdf


pdf: $(BASENAME).tex $(FIGURES) $(STYLEFILES)
	pdflatex -shell-escape $(BASENAME).tex
	bibtex $(BASENAME)
	pdflatex  -shell-escape $(BASENAME).tex
	pdflatex  -shell-escape $(BASENAME).tex
	@echo "\033[91m\n\n---------------------------------------\033[0m"
	@echo "\033[92mtarget \033[91m$(BASENAME).$@ \033[92mfinished successfully\033[0m"
	@echo "\033[91m---------------------------------------\n\033[0m"

zip:
	make clean
	tgz $(BASENAME).tgz Makefile *.*


clean:
	@rm -f  *~  
	@rm -f  *.aux *.bbl *.blg *.dvi *.log  *.pdfsync  *.ps *.tpt *.tgz
	@rm -f $(BASENAME).pdf 
	@rm -f  *~
	@echo "\n\033[92mtarget clean finished\n\033[0m" 
show:
	evince $(BASENAME).pdf

force: 
	touch $(BASENAME).tex
	make pdf

AD: appendix

appendix: AD.pdf

AD.pdf: AD.tex
	pdflatex AD.tex


==> XX_future.tex <==
\section{Discussion and beyond this paper} 
\label{sec:beyond}

In this paper, we focused on application-level characterization and hence we studied a single signal (total bandwidth) 
composed of I/O accesses coming from different processes. 
Nonetheless, there are situations where one could be interested in processes' behaviors, 
for example, for cache management (e.g. burst buffers). 
Note that our approach would work the same when applied at different levels. 
Similarly, our discussion on the selection of the sampling frequency (see Section~\ref{sec:param}) 
assumes that we are interested in \emph{any} frequency the application presents. 
When using the obtained information for techniques such as I/O scheduling, we may \emph{not} be interested in high 
frequencies (I/O phases that happen too fast and too often) because there is no time to do something about them. 
In that case, %saying the application just does I/O all the time would be a good-enough characterization, 
%and thus 
the sampling frequency could be selected as fast enough to capture the relevant frequencies.



% \begin{figure}
%     \centering
%     \includegraphics[width=0.48\textwidth]{images/illu_resolution.png}
%     \caption{Overview of resolution over time and frequency with different technics presented}
%     \label{fig:resolution}
% \end{figure}
% \at{change and extend}
% DFT transformation results in loss of the time information. That is, though DFT delivers accurately (depending on the sampling) the frequencies which constitute a signal, the exact occurrences of the frequencies is missing (time information). 
%The STFT gives could gives us a better resolution on time or frequency but we need to find the right time window for it to work. A wide window give a bad time resolution but a high frequency resolution. However, a short window gives good time resolution but we loose information on frequency.
% The wavelets transformation\cite{388960} overcomes this limitation, however, at a price for accuracy in the frequency domain. 
% This can be easily shown via Heisenberg Boxes (i.e., Time-Frequency uncertainty principle). On a plot showing the frequency versus time, DFT discretizes the frequency into bins (see \cref{eq:freq}). In contrast, all bins have the same length on the time axis, which is namely the time window. Hence, DFT has a high frequency resolution. In contrast, the wavelet transformation compromises this aspect. It results for low frequencies in short uncertainty boxes which are wide in the time domain and for high frequency in uncertainty boxes which are tall in the frequency domain and narrow in the time domain. This is good, as low frequency signals tend to last long in the time domain, hence a high time resolution is unnecessary. In contrast, high frequencies tend to last only for a short amount of time, hence, a high time resolution is necessary.    


% add more: \href{https://inst.eecs.berkeley.edu/~ee123/fa12/Notes/Lecture10.pdf}{link}

Still, the length of the time window impacts the resolution on the frequency domain 
(as discussed in Section~\ref{sec:param}).
%Fran - changed it to link better with the previous paragraph where we say we could not case about high frequency
%There are several limitations associated with predicting the I/O of 
%an application when using DFT which are associated with the parameter selection (see Section~\ref{sec:param}). 
%
% For example, as long as the I/O behavior is 
% repetitive, a dominant frequency can be extracted thus allowing to predict the 
% periodicity of the signal. However, I/O variations during the inspected time window can make it sometimes difficult to find the dominant frequency. This can be traced back to the fact that DFT transformation results in loss of the time information. That is, though DFT delivers accurately (depending on the sampling) the frequencies which constitute a signal, the exact occurrences of the frequencies is missing (time information). 
% Thus, it's quite well suited to 
% identify if a signal is periodic or not in a given time window, however, the selection 
% of the time window as well as significant I/O variations inside the window, can make the
% prediction inaccurate. Another source of inaccuracy is the sampling frequency. The selection of a high sampling frequency $f_s$ results in large number of samples $N$, which again result in (1) large calculation overhead and (2) in frequency spectrum with high precision. While the second part sounds like a advantage, it can be is some cases a disadvantage: Usually we are not interested in short I/O behavior (high frequency), which is why it's not worth the excessive overhead. However, to obtain accurate predictions (i.e. to capture the dominant frequency), a adequate sampling frequency is often required to avoid aliasing. Hence, a too low frequency is also no suited. 
%
Ideally, we desire a high resolution for the low frequencies and a low resolution for the high frequencies, 
%Ideally, we desire a high frequency resolution for the low frequencies and a low frequency resolution for the high frequencies, 
as we are focusing on I/O phases. %, where we are more interested in the lower frequencies behaviors. Fran - said it in the previous paragraph
Thus, it would be useful to have a multi-resolution scheme, which brings us to the wavelet transformation~\cite{388960}.
It overcomes the limitations of DFT, however, at a price for accuracy in the frequency domain. 
It could be used to improve the results of DFT (e.g., filtering high frequencies out), or as a standalone (instead of DFT). 
For the example in Section~\ref{sec:results} with 9216 ranks, we performed the continuous wavelet on the signal. 
The result for a decomposition level of three is shown in \cref{fig:dwt}. 
% As the sampling frequency was 10~Hz, a decomposition level of 10. %states that wavelet classifies the signal into three chunks: From 5 to 2.5~Hz, from 2.5 to 1.25~Hz, and from 1.25 to 0~Hz. 
The color scale on the right of \cref{fig:dwt} shows how present a particular frequency is at a given time in the signal (i.e., the amplitude of the wavelet coefficients). 
\begin{figure}[hbpt]
    \centering
    % \includegraphics[width=\columnwidth]{images/dwt.png}
    \includegraphics[width=\columnwidth]{images/9216_dtw_cont.png}
    \caption{Continous wavelet transformation on IOR with 9216 ranks with a decomposition level of ten. }
    \label{fig:dwt}
\end{figure}
We can clearly see the I/O phases as the red regions in \cref{fig:dwt}. 
Unlike DFT, the evaluation of the wavelet transformation needs more sophisticated methods (with heavier overhead) 
than those used here, which is why we left it out for future work. 

% \fb{the text says decomposition level of 3 and then there is an incomplete phrase saying decomposition level of 10. I don't understand it.}
% AT: used to e the discrete wavlet with level=3

% \at{speak about attaching to existing monitoring solution}
%Fran -moved it to conclusion


==> ideas.tex <==
\ideas{future todos: for SC23
\begin{itemize}
\item  outlier to see if regular or irregular 
\item bound memory fixed buffer size (compression) number of frequencies
\item look back into time with the predicted frequency and carry one the time window from this point, Make offline calculation with entire time window for comparison. Two metrics:one metric quantifies the similarity to the original signal (quality), and a second one confident interval (how many times you have frequency hit) 
- abstraction of bandwidth (bin size) to reduce sample frequency.\\
\item memory bound: maximum size is size(b)*size(double) + size(t)* size(double). abstract points based on size (remove short time or short bandwidth changes)
\end{itemize}
}

\ideas{
\begin{itemize}
    \item conference: CCGrid? PASC (December 11)? ISC (December 23)? SPAA (January)? Europar (January)?
    \item DFT allows us to find out the application's period
\item predict next i/o phases
\item there are a lot of parameters that affect how good the prediction is
\item what is the perfect sampling rate?
\item how to determine the good time window? too long has too much overhead, too small does not allow for seeing the signal correctly
\item what if the application behavior changes? how to we detect it? (with spill for the second paper)
\item what is noise? If the frequency is super high, we don't see it, but is it noise? what is the difference between that and a signal where there is no I/O happening?
\item length of the pattern is most important contribution. Everything else can be measured
\item wavelets provide range. Use it to find the sampling frequency and then DFT to find the exact one. 
\item volume of I/O when I/O is changing frequent
\item how precise it is and what is based on (what affects the precision)
\item evalute DFT: either using the wavlets (since it knows the time and when frequency occured) than compute area with wavlets to the specific period from DFT. and apply formula from the paper. directly the formula and see the smalles one.
\end{itemize}
}

\ideas{Proposition for structure of the paper
\begin{enumerate}
    \item Sec Motivation: Compact representation of IO behavior. Trade-off between compactness, simplicity and precision
    \item Sec Compact model: describe what we need (frequency/peak/confidence)
    \item Sec Algorithmic approach: Essentially Section~\ref{subsec:DFT}, maybe also wavelet section?
    \item Sec Evaluation + limits: 
    \begin{itemize}
        \item Comparison Wavelets/FFT: wavelets are a baseline
        \item Real Workload, show that we can obtain something
        \item Simulated workload: see the impact of a real system
        \begin{itemize}
            \item limits for irregular pattern
        \end{itemize}
    \end{itemize}
\end{enumerate}
}


==> iosetsapps.tex <==
\section{Test}

(this is not supposed to stay here, it's just a test, I'm putting this data here so we can see if we keep these results, and then we can decide where to put them and how to show them)

We show two examples from the same execution of this experiment: applications 2 and 10. Despite the fact that they were both designed to be periodic in isolation (with a period of 384s), their I/O phases are slowed down by other concurrent applications and by the I/O scheduler's decisions, and hence vary in duration. Tables~\ref{tab:iosets_app2} and~\ref{tab:iosets_app10} show the predictions obtained after each of these applications' 8 I/O phases: ``Period'' corresponds to the length of each iteration, ``Avg.'' shows the average iteration length so far, ``Pred.'' is the FTIO prediction, and ``Error'' compares each prediction with the current average. After the first iteration, FTIO is able to provide good estimates for the period, even under I/O variation that makes these applications deviate from periodic.

\begin{table}[!h]
\caption{Application 2}
\label{tab:iosets_app2}
\begin{tabular}{ccccccccc}
\textbf{Iter.}         & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} \\
\textbf{Period}     & 504      & 387      & 387      & 418      & 422      & 404      & 423      & 403      \\
\textbf{Avg.} & 504      & 445      & 426      & 424      & 424      & 420      & 421      & 418      \\
\textbf{Pred.}        & 127      & 507      & 450      & 439      & 433      & 428      & 428      & 424 \\
%\textbf{Period}     & 503.8      & 386.9      & 387.5      & 418.0      & 421.7      & 403.9      & 422.9      & 403.2      \\
%\textbf{Avg.} & 503.8      & 445.4      & 426.1      & 424.1      & 423.6      & 420.3      & 420.7      & 418.5      \\
%\textbf{Pred.}        & 126.7      & 506.8      & 449.8      & 439.0      & 432.7      & 427.6      & 428.2      & 424.3 \\
\textbf{Error}             & 75\%       & 14\%       & 5.5\%      & 3.5\%      & 2.1\%      & 1.7\%      & 1.8\%      & 1.3\%     
\end{tabular}
\end{table}
%all confidence > 0.99
%last prediction:
%[PREDICTOR]: P(periodic) = 100.000%
%[PREDICTOR]: P([0.001,0.002] Hz) = 87.50%
%[PREDICTOR]: |-> [0.001,0.002] Hz = [407.643,704.100] sec
%[PREDICTOR]: '-> P([0.001,0.002] Hz | perodic) = 87.50%


\begin{table}[]
\caption{Application 10}
\label{tab:iosets_app10}
\begin{tabular}{ccccccccc}
\textbf{Iter.}  & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} \\
\textbf{Period}     & 604      & 540      & 475      & 413      & 408      & 420      & 421      & 431      \\
\textbf{Avg.} & 604      & 572      & 540      & 508        & 488      & 477      & 469      & 464      \\
\textbf{Pred.}  & 190      & 704      & 599      & 536      & 501      & 484      & 408      & 411      \\
\textbf{Error}      & 68\%       & 23\%       & 11\%       & 5.4\%      & 2.7\%      & 1.5\%      & 13\%       & 11\%    \\
%\textbf{period}     & 603.9      & 539.8      & 475.1      & 413.3      & 408.4      & 420.2      & 421.5      & 431.3      \\
%\textbf{avg period} & 603.9      & 571.8      & 539.6      & 508        & 488.1      & 476.8      & 468.9      & 464.2      \\
%\textbf{predicted}  & 190.5      & 704.1      & 599.4      & 535.6      & 501.5      & 484.1      & 407.6      & 411.1      \\
%\textbf{error}      & 68\%       & 23\%       & 11\%       & 5.4\%      & 2.7\%      & 1.5\%      & 13\%       & 11\% 
\end{tabular}
\end{table}
%all confidence > 0.95
% last prediction:
%[PREDICTOR]: P(periodic) = 100.000%
%[PREDICTOR]: P([0.001,0.002] Hz) = 87.50%
%[PREDICTOR]: |-> [0.001,0.002] Hz = [407.643,704.100] sec
%[PREDICTOR]: '-> P([0.001,0.002] Hz | perodic) = 87.50%
%(it's not a mistake, it's exactly the same numbers as for app 2)

(here is a bad one in case we want to also show it: \ref{tab:iosets_app5})

\begin{table}[!h]
\caption{Application 5. ``-'' denotes ``non-periodic''.}
\label{tab:iosets_app5}
\begin{tabular}{ccccccccc}
\textbf{Iter.}  & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} & \textbf{8} \\
\textbf{Period} & 508        & 472        & 415        & 409        & 422        & 410        & 422        & 427        \\
\textbf{Avg.}   & 508        & 490        & 465        & 451        & 445        & 439        & 437        & 435        \\
\textbf{Pred.}  & 137        & 588        & 508        & 472        & 460        & -          & -          & -          \\
\textbf{Error}  & 73\%       & 20\%       & 9.1\%      & 4.7\%      & 3.3\%      &           &           &          
\end{tabular}
\end{table}

%\begin{table}[]
%\caption{Repetition 5, application 15}
%\begin{tabular}{cccccccc}
%\textbf{iteration}  & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} & \textbf{7} \\
%\textbf{period}     & 652.6      & 562.4      & 532.6      & 507.9      & 462.4      & 532.7      & 536.6      \\
%\textbf{avg period} & 652.6      & 607.5      & 582.5      & 563.9      & 543.6      & 541.8      & 541.0      \\
%\textbf{predicted}  & 188.9      & 735.3      & 637.1      & 597.4      & 564.4      & 465.6      & 475.1      \\
%\textbf{error}      & 71\%       & 21\%       & 9.3\%      & 5.9\%      & 3.8\%      & 14\%       & 12\%      
%\end{tabular}
%\end{table}

==> out.tex <==
\clearpage
\at{Check if contains something still needed}
\color{gray}
\paragraph{\textbf{Results interpretation}}
The result of DFT on the signal can then be visualized in the
frequency domain, where the frequencies $f_k$ (or frequency bins $k$) are plotted
against their corresponding amplitudes $|X_k|$.
%This visualization is called a periodogram.
\begin{figure}[h]
    \centering
    \includegraphics[width=\columnwidth,trim= 0 0 0 0cm, clip]{images/384_ior.png}
    % /Lichtenberg/git/ior/sim_sc23/sim2_100Hz
    \caption{Running example: IOR with 384 ranks.} % executed on the \machine cluster.}
    \label{fig:Running_example}
\end{figure}
As a running example, and to demonstrate the extraction of period from a signal, 
\at{cutted description}
The temporal I/O behavior is shown in \cref{fig:Running_example}. 
\ifextended
Unlike the example in Section~\ref{sec: motivation} (Figure~\ref{fig:mot_ior_1536}), 
we avoided the collective mode, as it is usually easier to characterize due to more consistent I/O phases and typically lower bandwidth. 
\fi
\begin{figure}[bpt]
    \centering
    \includegraphics[width=\columnwidth,trim= 0 0 0 0, clip]{images/384_bode.png}
    % /d/Lichtenberg/git/ior/sim_sc23/sim2_100Hz
    \caption{Two-sided frequency spectrum from DFT for IOR with 384 ranks and a sampling frequency set to 100 Hz.}
    \label{fig:ior_384}
\end{figure}
The result of DFT on this signal with $f_s=100$~Hz is shown in
\cref{fig:ior_384}, where the amplitudes $|X_k|$ are plotted against the frequencies $f_k$ for $k\in[0,N)$ (i.e., two-sided spectrum).
% For sake of completeness, we show the full frequency
%spectrum in this figure. As it is symmetric (see Section~\ref{subsec:DFT}), in
%the rest of this work, we only show the single-sided. \todo{No. no need to
%discuss this anymore.}

The amplitudes in the figure show the contribution of the frequencies to the
signal:
the higher the amplitude $|X_k|$, the more the frequency at $f_k$ 
contributes to the discretized signal $x_n$. This becomes especially interesting
when one signal has a significantly higher amplitude than the others. If this is
the case, the frequency of this signal (at $f_k$) delivers the periodicity of the I/O phases as it is the dominating one. As shown in \cref{fig:ior_384}, 
7605 (3803 for single-sided) frequencies contribute to the original signal. 
So the question is: How can we extract the dominating frequency, 
%that depicts the I/O periodicity, %of the signal 
if there is any?
% Hence, the task of finding the periodicity of the signal narrows to finding the frequency with the highest amplitude that is at the same time an outlier.


According to Section~\ref{subsec:DFT}, it is enough to examine half the spectrum (i.e., $\frac{N}{2}$). 
Hence, we look into the single-sided spectrum which plots the amplitude of only half the data against the frequency. 
However, the amplitudes are adjusted: $2|X_k|$ for $1\leq k \leq \frac{N}{2}$ and $|X_0|$ for $k=0$.
% shown in \cref{fig:ior_384}, however, the amplitudes need to be adjusted (i.e., symmetric values need to be multiplied by 2), as \cref{eq:simplefied_dft} depicts. 
\begin{figure}[tbhp]
    \centering
    \includegraphics[width=\columnwidth,trim= 0 0 0 0,clip]{images/ior_384_half_spectrum_zoom.png}
    % \at{hidden to save compile time}
    \caption{Single-sided spectrum from DFT on IOR with 384 ranks and a sampling frequency set to 100 Hz.}
    \label{fig:ior_384_half_spectrum}
\end{figure}
This is shown in \cref{fig:ior_384_half_spectrum}, %where the single-sided is illustrated 
for the running example from \cref{fig:Running_example}. 
We added a color scale that shows the contribution of the amplitude to the aggregate amplitude over the $\frac{N}{2}$ frequencies. 
Higher values are closer to yellow while lower values are closer to dark purple.
Since we set the sampling frequency $f_s=100$~Hz, and we are looking at the single-sided spectrum, 
one can expect to see frequencies up to 50~Hz. 
% no significant info is included in freq above 50 Hz -> nyquist
However, as the contribution of the frequencies up to 50~Hz is very low, we show only those up to 1.5~Hz. 
Moreover, the step between two consecutive frequencies is 0.013~Hz corresponding to $\frac{1}{\Delta t}$ ($\Delta t$ = 76.05~s).
As shown in \cref{fig:ior_384_half_spectrum}, the contribution of the component at $f_{0}=0$~Hz is the highest. 
%This was not only observed in this example but for several others examples as will be seen in Section~\ref{sec:results}. 
\ifextended
This observation makes sense, as I/O phases always transfer a 
positive (zero or above) number of bytes, and the cosine waves obtained with DFT need to be 
shifted upwards by an offset to reconstruct the signal. Shifting the signal upwards is the role of the 
component at $f_0$ (i.e., the DC offset), which is why it should be one of the highest contributing frequencies. 
Moreover, if this value is divided by the number 
of samples $N$, the arithmetic average is obtained. 
\else
aligning with what has been stated at the beginning of this section.
\fi

% Moreover, the spent effort (i.e., sampling frequency), the results might change as Section~\ref{sec:param} shows later . 
For the running example, 
\ifextended 
(from \cref{fig:ior_384_half_spectrum}) 
\fi
\begin{figure}[bthp]
    \centering
    \includegraphics[width=\columnwidth,trim= 0 0 0 0cm,clip]{images/ior_384_top_4.png}
    %freq_dft -freq=100 /d/Lichtenberg/git/ior/sim_sc23/sim2_100Hz/384.json
    \caption{The cosine waves of the frequencies with the top four amplitudes (including $f_0$) plotted against time. 
    The reconstructed signal, from all values, is also shown.}
    \label{fig:ior_384_top_5}
\end{figure}
we plotted the top four signals with the largest amplitudes (including $f_0$) in \cref{fig:ior_384_top_5}. %Fran - my latexmk is bugged and cref gives section 3.2 instead of the correct reference to a figure %Guillaume: I see undefined ref if I use your label
The figure contains the discretized signal (zoomed) with $f_s=100$~Hz which is identical to the reconstructed signal (obtained from the IDFT). 
To show the contribution of a frequency, we extracted its corresponding component from \cref{eq:simplefied_dft} with ($t = nT_s$ and a zero-order hold)
That is, the amplitudes of the cosine waves are $\frac{2X_k}{N}$ for $k\in[1,\frac{N}{2}$] and $\frac{X_k}{N}$ for $k=0$. 
Besides the offset at $f_0$, the frequency at $f_7=0.09$~Hz has the second-largest amplitude with a period of $\frac{1}{f_7}=10.86$~s.
% depicts the period of the signal. 
% as previously stated. 
%
As mentioned earlier, 80 frequencies had a Z-Score larger than 3.
By evaluating \cref{eq:maxzk}, only the Z-score of a single frequency at 0.09~Hz %, %(i.e., a period of 10.86 s) 
%corresponding to the frequency bin 
($k=7$) 
satisfies the equation. 
Hence, $f_d=f_7$ and the 
the period of I/O phases is 10.86~s with high confidence, which is shown in  
\cref{fig:ior_384_res}.
Note that the first I/O operation starts at $t=3.5s$. 
%, where we extracted the component at $k=7$ from the 
%IDFT (\cref{eq:simplefied_dft}) and plotted it against the discrete-time (i.e., over $n*T_s$). 
% AT: discrete time makes it complicted. 
\begin{figure}[!t]%[bhp]
    \centering
    \includegraphics[width=\columnwidth,trim= 0 0 0 0cm,clip]{images/ior_384_res.png}
    \caption{Result of our approach: The I/O behavior (blue) for the running example is periodic with a period of 10.86~s (i.e., $f_7=0.09$~Hz) as depicted by the signal in green.}
    \label{fig:ior_384_res}
\end{figure}


